Benchmarks Underestimate the Readiness of Multi-lingual Dialogue Agents

Creating multilingual task-oriented dialogue (TOD) agents is challenging due to the high cost of training data acquisition. Following the research trend of improving training data efficiency, we show for the first time, that in-context learning is sufficient to tackle multilingual TOD. To handle the challenging dialogue state tracking (DST) subtask, we break it down to simpler steps that are more compatible with in-context learning where only a handful of few-shot examples are used. We test our approach on the multilingual TOD dataset X-RiSAWOZ, which has 12 domains in Chinese, English, French, Korean, Hindi, and code-mixed Hindi-English. Our turn-by-turn DST accuracy on the 6 languages range from 55.6% to 80.3%, seemingly worse than the SOTA results from fine-tuned models that achieve from 60.7% to 82.8%; our BLEU scores in the response generation (RG) subtask are also significantly lower than SOTA. However, after manual evaluation of the validation set, we find that by correcting gold label errors and improving dataset annotation schema, GPT-4 with our prompts can achieve (1) 89.6%-96.8% accuracy in DST, and (2) more than 99% correct response generation across different languages. This leads us to conclude that current automatic metrics heavily underestimate the effectiveness of in-context learning.

==> evaluation.tex <==
\section{A Novel Evaluation Methodology}
The original experiment with mBart model in the X-RiSAWOZ paper uses both turn by turn evaluation that use the gold data of all the previous turns and subtasks as input, as well as end-to-end evaluation which uses model output from the previous subtask as the input for the next subtask. With GPT-4, we focus on turn by turn evaluation.\\
For the DST subtask, we use the exact-match (EM) with the label as evaluation after applying post-processing to the inference output. Post-processing ensures that (1) the domains and slots in the output are in lexical order and (2) slot values are canonicalized so that they lexically match those in the ontology. If canonicalization fails, we consider the output not an exact-match as database query would fail.\\
DST subtask also has strict conventions on which entities to include and which ones not to include. The belief state should only include slots that are agreed upon and confirmed by both user and the agent. So if the output contains slots that users are merely querying about and have not confirmed, we classify it incorrect, as the query result will be different from the gold label. \\
The output for the ACD subtask is either yes or no, so the exact match is used for evaluation. For DAG subtask, X-RiSAWOZ originally used EM as the metric, but there could be multiple correct dialogue acts to the given belief state and query result so EM does not accurately gauge the performance of the model. [TODO: new evaluation metric for DAG]\\
Lastly for the RG subtask, we want to evaluate the quality of the response generated. In the X-RiSAWOZ paper, BLEU score was used to measure the similarity with the gold response. However, we observe with GPT-4 that the quality of the generated response is often better than the gold label. [TODO: new evaluation metric for RG]\\
We also take all the errors from 250 samples for each subtask and perform manual error analysis for DST and DAG. 

==> limitation.tex <==
\section*{Limitations}
Given that our results rely on large language models, we expect the quality of our dialogue agent to be limited by the quality of the underlying LLM. Specifically, it is likely that there will be a significant drop in quality when this work is evaluated on truly low-resource languages, but unfortunately, we are not aware of any such TOD datasets.
Another limitation is that we experiment with \xrisawoz which uses slot-values, as opposed to more complex representations like SQL, or less common representations like TreeDST~\cite{cheng-etal-2020-conversational}, dataflow~\cite{dataflow} or ThingTalk~\cite{lam2022thingtalk} which LLMs might not be familiar with.
In addition, \xrisawoz has relatively limited inter-domain dependencies (e.g. complex ``parameter passing'' between APIs in different domains), which may make the task simpler than some real-world applications require.
Designing representation for TOD subtasks that are both more expressive and suitable for use with LLMs is a promising direction for future work.

